Subbotin Graphical Models for Extreme Value Dependencies with Applications to Functional Neuronal Connectivity

With modern calcium imaging technology, activities of thousands of neurons can be recorded in vivo. These experiments can potentially provide new insights into intrinsic functional neuronal connectivity, defined as contemporaneous correlations between neuronal activities. As a common tool for estimating conditional dependencies in high-dimensional settings, graphical models are a natural choice for estimating functional connectivity networks. However, raw neuronal activity data presents a unique challenge: the relevant information in the data lies in rare extreme value observations that indicate neuronal firing, rather than in the observations near the mean. Existing graphical modeling techniques for extreme values rely on binning or thresholding observations, which may not be appropriate for calcium imaging data. In this paper, we develop a novel class of graphical models, called the Subbotin graphical model, which finds sparse conditional dependency structures with respect to the extreme value observations without requiring data pre-processing. We first derive the form of the Subbotin graphical model and show the conditions under which it is normalizable. We then study the empirical performance of the Subbotin graphical model and compare it to existing extreme value graphical modeling techniques and functional connectivity models from neuroscience through several simulation studies as well as a real-world calcium imaging data example.

==> outline.tex <==

\section{Introduction}



\begin{itemize}
    \item Undirected graphical models are used in a wide variety of fields for unsupervised multivariate analysis.
    \item Special data sets/research questions - extreme values carry much more importance than non-extreme values; indicator of spikes.
    \item Example: graphical models for neuroscience - commonly used on fluorescence trace data to construct estimates of functional connectivity.
    \item Lit review: graphical model methods and data pre-processing methods for neuroscience/other extreme value data.
    \item Introduce a graphical model method for these types of situations. New graphical model distribution that more heavily weighs extreme values.
\end{itemize}

\section{Extreme Graphs}

Let $\XX  \in \mathbb{R}^{n \times p}$ be a data matrix.
\begin{itemize}
    \item Introduce $\ell_p$ norm, univariate generalized normal/Subbotin distribution.
    \item Introduce multivariate conditional distribution.
    \item Derive multivariate distribution. 
    \item Algorithms.
\end{itemize}


\section{Estimation and Selection}

\section{Simulation Study}


\begin{itemize}
    \item Simulate a network from the multivariate Subbotin.
    \item Simulate a network from a multivariate mixture model distribution with extreme value mode and non extreme mode.
\end{itemize}

\section{Empirical Data Study}

\begin{itemize}
    \item Fluorescence trace data in neuroscience.
    \item Estimate NS vs. ENS network.
    \item Compare overall graphs,
    \item Pick out a coupld of particular nodes that are similar + show node neighbors; see if firing at same time or not.
\end{itemize}

\section{Discussion}

==> spare.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{thm}[\textbf{Neighborhood Selection Consistency}]  \label{subbotinneighconsis} Consider the Extreme Lasso program with Subbotin distributed error. We require the following assumptions:

\begin{enumerate}
    \item Restricted strong convexity and Lipschitz continuity: The Fisher information matrix $Q_{S_iS_i}$ for the true support set $S_i$ has bounded eigenvalues, i.e. there exists some $E_{min} > 0$ and $E_{max} > 0$ such that $$E_{max} > \Lambda_{\min}(Q_{S_iS_i}) > E_{min}.$$ 
    \item Incoherence: There exists a constant $\alpha >0$ such that $$\|Q_{S^c S}Q_{SS}^{-1}\| < 1-\alpha.$$
\end{enumerate}

\noindent Consider the family of regularization parameters $$\lambda \geq  \frac{4 \kappa_{\text{IC}}}{\tau} \gamma \sqrt{ \frac{\log p}{n}} \bigg[    2 \sqrt{ \frac{2}{\gamma}}   +   \sqrt{ \frac{\log p}{n}}   \bigg].$$ Then, the following properties holds with probability greater than   $1 - c_1 \exp(- c_2 n \log p)$: 

(i) The Lasso has a unique solution with support contained
within $S$. (i.e., $S(\hat \beta) \subset S(\beta^*)$.

(ii) If $\min_{a \in S} | \beta^{*}_{a}| > (\frac{\tau}{\kappa_{\text{IC}}} \cdot \frac{1}{4} + 1 ) \cdot \frac{2\sqrt{s}}{\kappa_{ \Ell}} \cdot \frac{4 \kappa_{\text{IC}}}{\tau} \gamma \sqrt{ \frac{\log p}{n}} \bigg[    2 \sqrt{ \frac{2}{\gamma}}   +   \sqrt{ \frac{\log p}{n}}   \bigg],$ the lasso estimator is also sign consistent: $\text{sign} (\hat \beta_S) = \text{sign} (\beta^{*}_S)$.
\end{thm} 

With the result from Theorem 2, we can show that Algorithm 1 is a consistent estimator of the entire edge set of the graph and derive the performance guarantee for the full procedure by using a concentration bound. 

\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\subsection{Extreme Value Mixture Model}

We now study a simple case in which the both the extreme and Gaussian graphical models are misspecified with respect to the data generating process, but which can still produce observations with simultaneous rare extreme values in multiple variables. We generate data from a multivariate Gaussian mixture model distribution with a which has a small probability of generating contemporaneous extreme values at each observation. Specifically, the distribution is structured to have a single non-extreme Gaussian mode with a non-diagonal covariance matrix, as well as multiple extreme value modes which produce data points from a Gaussian distribution with a large positive mean for only a sparse subset of variables. Here, we define the true edges of the graph as all pairings between variables associated with the same extreme value mode; the resulting network resembles the sparse small world graph structure of the previous simulation. We generate $n = 10000$ observations and $p = 100$ variables from the mixture model distribution, and we set the probability of the occurrence of an extreme value mode at an average rate of 1 per 4000 observations.

We show the results of the mixture model simulation in Table \ref{tab:evmm}. The extreme graphical model performs the best out of all models. On the other hand, neither of the Gaussian graphical models nor the median quantile graphical model are able to accurately estimate the variables which are associated with the extreme value modes. This would appear to indicate that these methods are much less likely to capture the relationships with respect to the extreme value observations, instead finding the correlations with respect to the non-extreme mode of the Gaussian mixture distribution. For the quantile graphical model, the true positive and false discovery rates improve dramatically, as we increase the selected quantile. However, even at the 99.9th quantile, the extreme graphical model still performs considerably better than the quantile graphical model.

\begin{table}[H]
\centering
\caption{True positive rates and false discovery rates for the extreme value mixture model simulations.}
\label{tab:evmm}
\medskip
\begin{tabular}{l|r|r}
\hline
Model & TPR & FDR \\
 \hline
 NS & 0.1147 (0.0256)& 0.8840 (0.0241)\\
 Glasso & 0.1222 (0.0218)& 0.8733 (0.0222)\\
 \hline
 Quantile - 0.5 & 0.1069 (0.0415) & 0.9190 (0.0387)\\
 Quantile - 0.9 & 0.1591 (0.0429)& 0.8490 (0.0413)\\
 Quantile - 0.99 & 0.3702 (0.0494) & 0.6323 (0.0496)\\
 Quantile - 0.999 & 0.6333 (0.0456) & 0.3595 (0.0467)\\
 \hline
 Extreme NS & 0.9793 (0.0101) & 0.0215 (0.0116)\\
 \hline
\end{tabular}
\end{table}

\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[H]
\centering
\caption{True positive rates and false discovery rates for the joint multivariate generalized normal simulations.}
\label{tab:mvgn}
\medskip
\begin{tabular}{l|r|r}
\hline
Model & TPR & FDR \\
\hline
NS & 0.9014 (0.0302) & 0.0881 (0.0305) \\
Glasso &  0.9135 (0.0347) & 0.0739 (0.0368) \\
\hline
Quantile - 0.5 & 0.8948 (0.0435) & 0.0515 (0.0424) \\
Quantile - 0.9 & 0.5589 (0.0701) & 0.3908 (0.0667)\\
Quantile - 0.99 & 0.4390 (0.0683) & 0.5135 (0.0696) \\
Quantile - 0.999 & 0.2465 (0.0703) & 0.7144 (0.0654) \\
\hline
Extreme NS & 0.9296 (0.0305) & 0.0758 (0.0373)\\
\hline
\end{tabular} 
\end{table}


\begin{table}[H]
\centering
\caption{True positive rates and false discovery rates for the balanced network simulations.}
\label{tab:bn}
\medskip
\begin{tabular}{l|r|r}
\hline
Model & TPR & FDR \\
 \hline
 NS & 0.4354 (0.0520) & 0.4757 (0.0595)\\
 Glasso & 0.4516 (0.0551)& 0.5254 (0.0593) \\
 \hline
 Quantile - 0.5 & 0.0887 (0.0591) & 0.9360 (0.0544) \\
 Quantile - 0.9 & 0.5693 (0.0854) & 0.4508 (0.0835)\\
 Quantile - 0.99 & 0.7580 (0.0951) & 0.2357 (0.0909)\\
 Quantile - 0.999 & 0.5754 (0.1276) & 0.4214 (0.1265)\\
 \hline
 Extreme NS & 0.8951 (0.0452) & 0.0891 (0.0484) \\
 \hline
\end{tabular}
\end{table}



%\begin{itemize}
    % \item Undirected graphical models are used in a wide variety of fields for unsupervised multivariate analysis.
    % \begin{itemize}
        %\item Genomics.
        %\item Network biology.
        %\item Finance, manufacturing.
    % \end{itemize}
    % \item Current research of interest: graphical models for neuroscience - commonly used on calcium imaging data to construct estimates of functional neuronal connectivity.
    %\begin{itemize}
        %\item Special type of data set/research question; because of nature of data, extreme values carry much more importance than non-extreme values - indicator of spikes.
        %\item Non-extreme values/0's are generally much less valuable information; mostly comprised of noise.
    %\end{itemize}
    %\item Lit review: graphical model methods and data pre-processing methods for neuroscience.
    %\begin{itemize}
     %   \item Denoising + deconvolution + thresholding/spike calling before using typical GGM.
      %  \item Issue: multi-step process involves error propagation.
    %\end{itemize}
    %\item Introduce a new graphical model method for these types of situations. 
    %\begin{itemize}
     %   \item Extreme graphical model.
     %   \item New graphical model distribution that more heavily weighs extreme values.
     %   \item Advantage: single step method, smooth loss function.
    %\end{itemize}
%\end{itemize}

\begin{comment}
\subsection{Estimation and Selection}

\begin{thm}[Joint Distribution of Multivariate Subbotin:]
Suppose ($X_1, X_2, \hdots , X_p$) is a p-dimensional random vector, and its node-wise conditional distributions are given by: $$f(\XX_i|\XX_{-i}) = \frac{1}{2\sigma\nu(\frac{1+\nu}{\nu})} e^{-((x_i - \sum_{j \neq i}\theta_{ij} x_{j}) / \sigma)^{\nu}}$$ for some even integer $\nu$.  Without loss of generality, let $\sigma = 1$ for all conditional distributions. Then, under the condition $$ \sum_{i = 1}^p \left(- (x_i - \sum_{j < i} \theta_{ij}x_j)^{\nu} + (\sum_{j < i} \theta_{ij}x_j)^{\nu} \right) > 0$$ for all $\XX \in \Rnp$, the joint distribution is given by $$f(\XX) = \exp \left(- \sum_{i = 1}^p \left(- (x_i - \sum_{j < i} \theta_{ij}x_j)^{\nu} + (\sum_{j < i} \theta_{ij}x_j)^{\nu} \right) - A(\boldsymbol{\Theta}) \right).$$ 
\end{thm} 

\medskip 
\noindent \textit{Proof:} Our proof of Theorem 1 is comprised of two parts. First, we formulate the functional form of the joint distribution explicitly. We then show that, under the stated positivity condition, the log normalization constant of the distribution $A(\theta)$ will be finite and positive for all $\XX \in \Rnp$ and therefore the distribution will exist.

\medskip
\noindent \textit{Functional Form:}  Our derivation of the functional form of the joint distribution follows from Besag (1974), which showed that a valid multivariate joint distribution can be derived from a known conditional distribution via the equivalency $$Q(\xx) = \prod_{i = 1}^p \frac{P(x_{i}|x_1, x_2, \hdots, x_{i-1}, y_{i+1}, \hdots y_p)}{P(y_{i}|x_1, x_2, \hdots, x_{i-1}, y_{i+1}, \hdots y_p )}$$ (Note that since the distribution is supported on the entirety of $\mathbb{R}^p$, the necessary assumption of a non-zero probability for all denominators is fulfilled.) We derive the exponential functional form of the joint distribution in Theorem 1 by defining $$Q(\xx) := \log(P(\xx) / P(\boldsymbol{0})),$$ which can be shown to be equivalent to $$Q(\xx) = \log \left(\prod_{i = 1}^p \frac{P(x_{i}|x_1, x_2, \hdots, x_{i-1}, y_{i+1} = 0, \hdots y_p = 0)}{P(y_{i} = 0|x_1, x_2, \hdots, x_{i-1}, y_{i+1} = 0, \hdots y_p = 0)}\right).$$ We then replace $Q(\xx)$ with the Hammersley-Clifford definition of the most general form of a graphical model joint distribution to get: $$ \sum_{1 \leq i \leq p} x_i G_i(x_i) + \sum_{1 \leq i \leq j \leq p} x_i x_j G_{ij}(x_i, x_j) + \hdots  = \log \left(\prod_{i = 1}^p \frac{P(x_{i}|x_1, x_2, \hdots, x_{i-1}, y_{i+1} = 0, \hdots y_p = 0)}{P(y_{i} = 0|x_1, x_2, \hdots, x_{i-1}, y_{i+1} = 0, \hdots y_p = 0)}\right).$$ For our particular case, there will be interaction terms in the Hammersley-Clifford form of the distribution up to the $\nu$-th order. We can then find equivalencies between individual terms on the left and right hand sides of the above equation. Without loss of generality, we first operate on $\xx_p.$ Define: $$\xx_{i:0} := (x_1, \hdots, x_{i-1}, 0, x_{i + 1}, \hdots, x_p).$$ By definition, we have $$\frac{\exp(Q(\xx))}{\exp(Q(\xx_{p:0}))} = \exp(Q(\xx) - Q(\xx_{p:0})) = x_p\left(G_p(x_p) + \sum_{1 \leq i \leq p-1} x_i G_{ip}(x_i, x_p)\right)$$ and $$\frac{\exp(Q(\xx))}{\exp(Q(\xx_{p:0}))} = \frac{P(\xx)}{P(\xx_{p:0})} = \frac{P(x_{p}|x_1, x_2, \hdots, x_{p-1})}{P(x_{p} = 0|x_1, x_2, \hdots, x_{p-1})}.$$ The two above equations allows us to isolate only those terms which are functions of $x_p$. The latter equation also gives us the first term of the product $\prod_{i = 1}^p \frac{P(x_{i}|x_1, x_2, \hdots, x_{i-1}, y_{i+1} = 0, \hdots y_p = 0)}{P(y_{i} = 0|x_1, x_2, \hdots, x_{i-1}, y_{i+1} = 0, \hdots y_p = 0)}.$ Specifically we get: 
\begin{eqnarray*}
    x_p\left(G_p(x_p) + \sum_{1 \leq i \leq p-1} x_i G_{ip}(x_i, x_p)  + \hdots\right) & = & \frac{P(x_{p}|x_1, x_2, \hdots, x_{p-1})}{P(x_{p} = 0|x_1, x_2, \hdots, x_{p-1})}\\
    & = & \exp\left(-(x_p - \sum_{i \leq p-1} \theta_{ip}x_i)^{\nu}  + (\sum_{i \leq p-1} \theta_{ip}x_i)^{\nu}\right) \\
\end{eqnarray*} Using arithmetic to expand the right hand side of the above equation, we can find each individual $G$ function: 
$$G_p(x_p) = - x_p^{\nu - 1}, $$ $$G_{ip}(x_i, x_p) =  - \theta_{ip} \left((x_p - \theta_{ip} x_i)^{\nu - 2} - (\theta_{ip} x_i)^{\nu - 1} \right),$$ \hspace{-0.5cm} $$ G_{ijp}(x_i, x_j, x_p) = - \theta_{ip} \theta_{jp} \left((x_p - \theta_{ip} x_i - \theta_{jp} x_j)^{\nu - 3}  - (\theta_{ip} x_i - \theta_{jp} x_j)^{\nu - 2} \right),$$  and so on, up to the $\nu$-th order $G$ function. One particular thing to note is that, if $\theta_{ip} = 0$, then all $G$ functions involving $x_i$ and $x_p$ will be equal to 0, meaning that this is a valid form for the joint probability distribution by the Hammersley-Clifford theorem. We can then operate recursively to get the $G$ functions for all $r \in 1, 2, \hdots, p$. For example, for $x_{p-1}$, we get: \begin{eqnarray*}
    x_{p-1}\left(G_{p-1}(x_{p-1}) + \sum_{1 \leq i \leq p-2} x_i G_{i(p-1)}(x_i, x_p)  + \hdots\right) & = & \frac{P(x_{p-1}|x_1, x_2, \hdots, x_{p-2}, x_p = 0)}{P(x_{p-1} = 0|x_1, x_2, \hdots, x_{p-2}, x_p = 0)}\\
    & = & \exp\left(-(x_p - \sum_{i \leq p-2} \theta_{ip}x_i)^{\nu}  + (\sum_{i 
\leq p-2} \theta_{ip}x_i)^{\nu}\right) \\
\end{eqnarray*} Putting all terms together for all variables, we get the following form of the joint distribution:
\begin{eqnarray*}
    Q(\xx) & = & \log \left(\prod_{i = 1}^p \frac{P(x_{i}|x_1, x_2, \hdots, x_{i-1}, y_{i+1} = 0, \hdots y_p = 0)}{P(y_{i} = 0|x_1, x_2, \hdots, x_{i-1}, y_{i+1} = 0, \hdots y_p = 0)}\right) \\
    & = & - \sum_{i = 1}^p \left((x_i - \sum_{j < i} \theta_{ij}x_j)^{\nu} - (\sum_{j < i} \theta_{ij}x_j)^{\nu} \right)\\
    f(\XX) & \propto& \exp(Q(\xx)) \\
    & \propto& \exp\left(- \sum_{i = 1}^p \left( (x_i - \sum_{j < i} \theta_{ij}x_j)^{\nu} - (\sum_{j < i} \theta_{ij}x_j)^{\nu} \right)\right).
\end{eqnarray*} 

\bigskip 

\noindent \textit{Log Normalizing Constant:} Typically, the normalizing constant of the joint distribution is found by finding the solution to the integral (written below in the case that we have assumed WLOG that $\boldsymbol{\mu} = \boldsymbol{0}$):
\begin{eqnarray*}
    A(\boldsymbol{\Theta})& = & \int_{-\infty}^{\infty}  \exp(Q(\xx)) d \xx \\
    & = & \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} \int_{-\infty}^{\infty} \hdots  \exp(Q(\xx)) d x_1 d x_2 d x_3 \hdots
\end{eqnarray*} For $\nu>2$, $A(\boldsymbol{\Theta})$ will usually not have a closed form solution. However, we show below that $f(\xx)$ will always be positive for all $\xx \in \Rp$ and that under certain conditions $A(\boldsymbol{\Theta})$ will be finite.

\medskip

\noindent \textit{Positivity:} Since $e$ is a positive number, $\exp(Q(\xx))$ will be positive as long as $Q(\xx)$ is a real number. This will always be the case for $\xx \in \Rp$ with the particular form of $Q(\xx)$ given for the multivariate joint distribution.

\medskip

\noindent \textit{Finiteness:} In order for $A(\boldsymbol{\Theta})$ to be finite, we require that $\exp(Q(x))$ have a finite integral. This can be guaranteed if and only if the parameters $\boldsymbol{\Theta}$ are such that $Q(x) < 0$ for all $\xx \in \Rnp$. Under this condition, we can show that the integral $\int_{-\infty}^{\infty}  \exp(Q(x_i | \xx_{-i})) d x_i$ is finite for all $i \in \{1, 2, \hdots, p\}$ in the following manner. Let $g(x_i) = -x_i^2.$ If $\nu>2$ and $Q(x) < 0$, then it is trivial to show that $$\lim_{x_i \rightarrow \infty} \frac{\exp(Q(x_i | \xx_{-i}))}{\exp(g(x_i))} = \lim_{x_i \rightarrow \infty} \exp(Q(x_i | \xx_{-i}) - g(x_i)) = 0.$$ Using the above, by the limit comparison theorem, we can say that if $\int_{-\infty}^{\infty} \exp(g(x_i)) dx_i$ converges, then $\int_{-\infty}^{\infty} \exp(Q(x_i | \xx_{-i})) dx_i$ converges as well. Analytically, it can be shown that $$\int_{-\infty}^{\infty} \exp(-x_i^2) dx = \sqrt{2 \pi},$$ so the integral converges. Thus, the integral $$\int_{-\infty}^{\infty}\exp(Q(x_i | \xx_{-i})) d x_i$$ will be finite as well. This will hold for each individual integral, as each individual component will have an independent integral. Thus, the full distribution is of the form 
\begin{eqnarray*}
    f(\XX) & = & \exp(Q(\xx) - A(\boldsymbol{\Theta})) \\
    & = & \exp\left(-\sum_{i = 1}^p \left( (x_i - \sum_{j < i} \theta_{ij}x_j)^{\nu} - (\sum_{j < i} \theta_{ij}x_j)^{\nu} \right) - A(\boldsymbol{\Theta}) \right).
\end{eqnarray*} where the distribution exists if and only if $$-\sum_{i = 1}^p \left( (x_i - \sum_{j < i} \theta_{ij}x_j)^{\nu} - (\sum_{j < i} \theta_{ij}x_j)^{\nu} \right) < 0$$ for all $\xx \in \Rnp$ for a particular $\boldsymbol{\Theta}$. \hfill \qedsymbol

\begin{itemize}
    \item Comment on independence if $\theta_{ij} = 0.$
\end{itemize}


\noindent Theorem from the Extreme Lasso paper:

\begin{thm}[\textbf{Neighborhood Selection Consistency for Subbotin Error}]  \label{subbotinneighconsis} Consider the Extreme Lasso program with Subbotin distributed error.  Assume that Assumptions 1-6 hold. Consider the family of regularization parameters $$\lambda \geq  \frac{4 \kappa_{\text{IC}}}{\tau} \nu \sqrt{ \frac{\log p}{n}} \bigg[    2 \sqrt{ \frac{2}{\nu}}   +   \sqrt{ \frac{\log p}{n}}   \bigg] $$, then the following properties holds with probability greater than   $1 - c_1 \exp(- c_2 \log p)$: 

(i) The Lasso has a unique solution with support contained
within $S$. (i.e., $S(\hat \beta) \subset S(\beta^*)$.

(ii) If $\min_{a \in S} | \beta^{*}_{a}| > (\frac{\tau}{\kappa_{\text{IC}}} \cdot \frac{1}{4} + 1 ) \cdot \frac{2\sqrt{s}}{\kappa_{ \Ell}} \cdot \frac{4 \kappa_{\text{IC}}}{\tau} \nu \sqrt{ \frac{\log p}{n}} \bigg[    2 \sqrt{ \frac{2}{\nu}}   +   \sqrt{ \frac{\log p}{n}}   \bigg],$ the lasso estimator is also sign consistent: $\text{sign} (\hat \beta_S) = \text{sign} (\beta^{*}_S)$.
\end{thm} 

\noindent We also require the following assumptions:
\begin{enumerate}
    \item Dependency/bounded eigenvalues: The Fisher information matrix has bounded eigenvalues, i.e. there exists some $E_{min} > 0$ and $E_{max} > 0$ such that $$E_{max} > \Lambda_{\min}(Q_{SS}) > E_{min}.$$ 
    \item Incoherence: There exists a constant $\alpha >0$ such that $$\|Q_{S^c S}Q_{SS}^{-1}\| < 1-\alpha.$$
\end{enumerate}

\begin{thm}[\textbf{Model Selection Consistency for Subbotin Error}]  \label{subbotinmodelconsis} Consider the Extreme Lasso program with Subbotin distributed error.  Assume that Assumptions 1 and 2 hold. Consider the family of regularization parameters $$\lambda \geq \frac{4 \kappa_{\text{IC}}}{\tau} \nu \sqrt{ \frac{\log p}{n}} \bigg[    2 \sqrt{ \frac{2}{\nu}}   +   \sqrt{ \frac{\log p}{n}}   \bigg] $$ and let $$n > L d^2 \log{p}$$ where $d$ is the maximum neighborhood size. Then, the following properties holds with probability greater than   $1 - c_1 \exp(- c_2 (\log p)^2)$: 

(i) The edge set has unique solution with support contained
within $S$. (i.e., $S(\hat E) \subset S(E^*)$.

(ii) If $\min_{a \in S} | E^{*}_{a}| > (\frac{\tau}{\kappa_{\text{IC}}} \cdot \frac{1}{4} + 1 ) \cdot \frac{2\sqrt{s}}{\kappa_{ \Ell}} \cdot \frac{4 \kappa_{\text{IC}}}{\tau} \nu \sqrt{ \frac{\log p}{n}} \bigg[    2 \sqrt{ \frac{2}{\nu}}   +   \sqrt{ \frac{\log p}{n}}   \bigg]$, then $\hat{E}$ is also sign consistent: $\text{sign} (\hat{E}) = \text{sign} (E^*)$.
\end{thm} 

\noindent \textit{Proof:} By Theorem 2, conditions (i.) and (ii.) hold for a single neighborhood with probability $$1 - c_1 \exp(- c_2 \log p).$$ This means that they do not hold with probability $$p c_1 \exp(- c_2 \log p).$$ Using a union bound, we get that the probability of any neighborhood not holding is less than $$p c_1 \exp(- c_2 \log p).$$ Thus, the probability for the entire graph will be: 
\begin{eqnarray*}
&& 1 - p c_1 \exp(- c_2 \log p) \\
& = & 1 - c_1 \exp(- c_2 (\log p)^2) \\
\end{eqnarray*} \hfill \qedsymbol

\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



In Figure \ref{fig:bn}, we compare examples of edges selected in one of the balanced network simulation replications. In the top part of Figure \ref{fig:bn}, we see an edge that was selected as a false positive from the estimate of the Gaussian graphical model but which was found as a true negative by the extreme graphical model estimate; in the bottom part of Figure \ref{fig:bn}, the particular edge shown is a true positive selected by the extreme graphical model estimate, but a false negative as per the Gaussian graphical model estimate. In the former case, the Gaussian graphical model has selected an edge between two variables which have not spiked contemporaneously, but rather which are correlated based on the added convolution noise. Thus, we can see that the Gaussian graphical model is susceptible to selecting edges based on the unimportant noise part of the data. On the other hand, in the latter case, we see that the extreme graphical model was able to correctly select as an edge a pair of variables which spike at the same observation time once, even though there are other spikes which do not match up. This shows that the extreme graphical model can find neurons with some correlated spiking activity, even if not all of the spikes for a pair of neurons are aligned.

\begin{figure}[H] 
    \caption{\textbf{Top:} Traces of a pair of neurons selected as a false positive by the Gaussian graphical model estimate and a true negative by the extreme graphical model estimate. \textbf{Bottom:} Traces of a pair of neurons selected as a false negative by Gaussian graphical model estimate and a true positive by the extreme graphical model estimate.}
    \label{fig:bn}
    \centering
    \medskip
    \includegraphics[scale = 0.75]{paper_bn_comp.jpeg}
\end{figure}

\begin{figure}[H] 
    \caption{\textbf{Top:} Trace of a single particular neuron (black) vs. trace of selected edge neighbor (red) as selected by Gaussian graphical model. \textbf{Bottom:} Trace of a single particular neuron (black) vs. trace of selected edge neighbor (red) as selected by extreme graphical model.}
    \label{fig:same}
    \centering
    \includegraphics[scale = 0.75]{paper_same.jpeg}
\end{figure}

We also show the differences in the edges selected for the same neuron in both graph estimates in Figure \ref{fig:same}; the top 2 trace pair plots shown estimated edges from the Gaussian graphical model,  while the bottom 2 plots show estimated edges from the extreme graphical model. Specifically, the neuron we highlight has a couple of neighbors in both estimated networks for the Gaussian and extreme graphical models, but the neighbors selected by each method are different. We can see from Figure \ref{fig:same} that the neighbors in the graph estimated by the Gaussian graphical model do not share any similar spiking patterns with the highlighted neuron. On the other hand, the same neuron and its neighbors as selected by the extreme graphical model appear to spike at the same time as one another at least once. From this example, the extreme graphical model seems to do a better job of finding neurons which share similar spiking patters, as is the goal when estimating functional neuronal connectivity networks. 

%%%%%%%%%%%%%%%%%%%

\begin{figure}[t] 
    \centering
    \medskip
    \includegraphics[scale = 0.7]{20_104.png}
    \includegraphics[scale = 0.7]{20_170.png}
    \caption{Trace of hub neuron (black) vs. traces of selected edge neighbors (red) in Gaussian graphical model functional connectivity estimate.}
    \label{fig:ns}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[scale = 0.7]{2_214.png}
    \includegraphics[scale = 0.7]{2_55.png}
    \caption{Trace of hub neuron (black) vs. traces of selected edge neighbors (red) in extreme graphical model functional connectivity estimate.}
    \label{fig:ens}
\end{figure}


$\boldsymbol{P}$ = $\boldsymbol{\Sigma}^{-1},$ i.e. $\boldsymbol{P}$ is the precision matrix of the distribution.

Estimating functional neuronal connectivity networks in the brain is of interest to researchers as it can help provide a better understanding how the brain processes information and how different parts of the brain communicate with one another \citep{bb1}. 

However, one notable challenge which arises when analyzing calcium imaging data is that the observations across time carry different amounts of importance. Specifically,


%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%




\begin{comment}

\subsection{Subbotin Graphical Model Distribution}

For our first set of simulations, we investigate the efficacy of our estimation procedure on the multivariate graphical model distribution from which it is derived. As a baseline simulation, we generate $n = 2000$ observations and $p = 100$ features from the Subbotin graphical model distribution as defined in Equation 3 with $\nu = 8$, using a Gibbs sampling procedure with the univariate node-wise conditional distributions as defined in Equation 2. The network parameter matrix $\boldsymbol{\Theta}$ is structured as a sparse small world graph with 5 total cliques. We compare the Subbotin graphical model for $\nu = 4, 6 $ and 8, the Gaussian graphical model estimated using neighborhood selection and the graphical Lasso, and the quantile graphical model at the 50th and 90th percentiles. We then vary the number of observations and features, the $\nu$ parameter of the Subbotin graphical model distribution, and the structure of the underlying graph and analyze how the performance of each method changes.

\begin{table}[t]
\caption{Average TPR, FDP. (std. devs) for multivariate Subbotin graphical model distribution simulations with oracle tuning, averaged over 5 replicates. Best performing methods are boldfaced.}
\label{tab:mvgn}
\bigskip
\begin{footnotesize}
\begin{tabular}{|l|r|r|r|r|}
    \cline{1-3}
    & \multicolumn{2}{|c|}{Baseline}  \\
    \cline{1-3}
    \textbf{Model} &TPR&FDP \\
    \cline{1-3}
    Extreme (4) & 0.793 (0.058) &  0.205 (0.059)  \\
    Extreme (6) & 0.812 (0.054) &  0.200 (0.050) \\
    Extreme (8) & \textbf{0.840} (0.052) &  \textbf{0.166} (0.053) \\
    \cline{1-3}
    Gaussian Glasso & 0.756 (0.053) & 0.238 (0.054)  \\
    Gaussian NS & 0.779 (0.061) & 0.215 (0.059) \\
    \cline{1-3}
    Quantile (0.5)  & 0.689 (0.075) & 0.223 (0.079) \\
    Quantile (0.9) & 0.277 (0.083) & 0.727 (0.087)\\
    \hline
     & \multicolumn{2}{|c|}{$n = 1000$} & \multicolumn{2}{|c|}{$n = 4000$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & 0.534 (0.058) &  0.469 (0.059) & 0.853 (0.052) & 0.150 (0.054) \\
    Extreme (6) & 0.564 (0.062) &  0.441 (0.060) & 0.859 (0.051) & 0.142 (0.053) \\
    Extreme (8) & \textbf{0.631} (0.055) &  \textbf{0.367} (0.053) & \textbf{0.893} (0.055) & \textbf{0.105} (0.055) \\
    \hline
    Gaussian Glasso & 0.497 (0.055) & 0.491 (0.054) & 0.854 (0.051) & 0.126 (0.054) \\
    Gaussian NS & 0.503 (0.059) & 0.490 (0.059) & 0.863 (0.048) & 0.125 (0.047)\\
    \hline
    Quantile (0.5) & 0.482 (0.079) & 0.520 (0.075) & 0.817 (0.071) & 0.172 (0.073)\\
    Quantile (0.9) & 0.259 (0.081) & 0.744 (0.084)& 0.345 (0.077) & 0.652 (0.075)\\
    \hline
    & \multicolumn{2}{|c|}{$p = 300$} & \multicolumn{2}{|c|}{$p = 1000$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & 0.684 (0.058) &  0.311 (0.056) & 0.503 (0.059) &  0.501 (0.060)  \\
    Extreme (6) & 0.732 (0.059) &  0.272 (0.055) & \textbf{0.563} (0.053) & \textbf{0.438} (0.056) \\
    Extreme (8) & \textbf{0.751} (0.056) &  \textbf{0.250} (0.054) & 0.545 (0.061) &  0.452 (0.055)  \\
    \hline
    Gaussian Glasso & 0.616 (0.050) & 0.388 (0.049) & 0.480 (0.053) & 0.518 (0.055) \\
    Gaussian NS & 0.634 (0.053) & 0.362 (0.056) & 0.471 (0.057) & 0.507 (0.055) \\
    \hline
    Quantile (0.5) & 0.573 (0.078) & 0.427 (0.081) & 0.416 (0.077) & 0.590 (0.078)  \\
    Quantile (0.9) & 0.265 (0.085) & 0.747 (0.085) & 0.284 (0.079) & 0.731 (0.082) \\
    \hline
    & \multicolumn{2}{|c|}{$\nu = 4$} & \multicolumn{2}{|c|}{$\nu = 6$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & \textbf{0.886} (0.053) &  \textbf{0.107} (0.054) & 0.823 (0.060) &  0.170 (0.059)  \\
    Extreme (6) & 0.842 (0.057) &  0.158 (0.055) & \textbf{0.855} (0.057) &  \textbf{0.137} (0.057)  \\
    Extreme (8) & 0.734 (0.062) &  0.261 (0.058) & 0.775 (0.051) &  0.218 (0.058) \\
    \hline
    Gaussian Glasso & 0.872 (0.053) & 0.122 (0.054)  & 0.827 (0.053) & 0.171 (0.054)   \\
    Gaussian NS & 0.865 (0.053) & 0.134 (0.050) & 0.779 (0.051) & 0.225 (0.059)  \\
    \hline
    Quantile (0.5) & 0.664 (0.072) & 0.335 (0.073)  & 0.626 (0.072) & 0.381 (0.079)  \\
    Quantile (0.9) & 0.252 (0.079) & 0.776 (0.081) & 0.250 (0.080) & 0.746 (0.083) \\
    \hline
    & \multicolumn{2}{|c|}{Chain} & \multicolumn{2}{|c|}{Erdos-Renyi} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & 0.696 (0.052) &  0.304 (0.059) & 0.644 (0.056) &  0.358 (0.057) \\
    Extreme (6) & 0.711 (0.054) &  0.290 (0.050) & 0.659 (0.054) &  0.346 (0.061) \\
    Extreme (8) & \textbf{0.733} (0.058) &  \textbf{0.271} (0.055) & \textbf{0.672} (0.061) &  \textbf{0.329} (0.057)  \\
    \hline
    Gaussian Glasso  & 0.653 (0.049) & 0.348 (0.051)  & 0.615 (0.052) & 0.238 (0.070) \\
    Gaussian NS & 0.667 (0.058) & 0.335 (0.056) & 0.629 (0.060) & 0.374 (0.059)\\
    \hline
    Quantile (0.5) & 0.569 (0.072) & 0.338 (0.071) & 0.556 (0.071) & 0.452 (0.073) \\
    Quantile (0.9) & 0.225 (0.083) & 0.786 (0.084) & 0.234 (0.086) & 0.768 (0.079) \\
    \hline
\end{tabular}
\end{footnotesize}
\end{table}

Table \ref{tab:mvgn} show the results of the simulations. In general, the extreme neighborhood selection algorithm is able to identify the true network structure of the Subbotin distribution with fairly high accuracy. We also see that the Gaussian graphical models and the median quantile graphical model performs relatively well in terms of model selection, while the quantile graphical model at the 90th percentile generally performs much worse. The former of these results are unsurprising; since the probability density function of the Subbotin graphical model distribution is still a symmetric bell-shaped curve around the location parameter, and because the overall empirical correlation structure of the generated distribution will still be very close true parameter matrix, we would expect the graphical models which fit toward the mean or the median to do well. On the other hand, sampling from the multivariate Subbotin distribution is unlikely to generate contemporaneous extreme values between two variables which are related in the parameter matrix, as it is a thin tailed distribution. Thus, the quantile graphical models with high quantiles are unlikely to estimate the true network structure well, which we see reflected in the results. Comparing the results for simulation parameters, we see that reducing the number of observations and increasing the number of features decreases the true positive rate for all methods, with a greater impact on the Gaussian graphical model in the former and the Subbotin graphical model in the latter. We also see that the Subbotin graphical model with the true $\nu$ always has the best performance, which we would expect. Finally, we see that the Subbotin graphical model does best for all the various types of graph structures, although the true positive rate decreases more severely for non-small world graphs.


\subsection{Artificial Neuronal Network}

We now investigate a simulation study which is based upon neuroscience applications. Here, we simulate data from the balanced network model of \citep{aa2}, which utilizes a neuronal spiking model in order to create data which emulates the physical processes which comprise functional neuronal connectivity. In particular, the balanced network generates correlated spiking patterns between variables over time, mimicking the behavior of neurons as observed during calcium imaging experiments. The output of the balanced neuronal network algorithm is a set of spike times for each neuron, which we denote as the set $$T = \{(i, j)| \text{ neuron } j \text{ spikes at time } i\}.$$ To replicate fluorescence traces from calcium imaging, we then simulate each neuron's activity as an AR(1) process with innovations at the times specified by $T$: $$X_{ij} = \alpha \XX_{i-1, j} + [\mathbbm{1}_{[(i, j)]}(T)]Z_{ij} + \epsilon_{ij}$$ $$Z \sim N(\mu, 1)$$ $$\epsilon \sim N(0, 1).$$ Here, we consider the true underlying graph to be comprised of edges which connect all pairs of simulated neurons which spike contemporaneously, i.e $$G = \{(j, k)|\, \exists \, i : (i,j) \in T \cap (i,k) \in T \}.$$ For this simulation study, we use as a baseline case $n = 5000$ time points for $p = 100$ simulated neurons, along with parameter values $\alpha = 0.5$ and $\mu = 20$. We also limit the spike rate of the variables such that spikes occur at a maximum of 0.001 Hz in order to emulate the rarity of the extreme values that are seen in real-world fluorescence trace data. We compare the Subbotin graphical model for $\nu = 4, 6 $ and 8, the Gaussian graphical model estimated using neighborhood selection and the graphical Lasso, and the quantile graphical model at the 50th, 90th, 99th, and 99.9th percentiles. We also vary the number of simulated neurons, the maximum spiking rate, and the average size of each spike in the simulations below.

\begin{table}[t]
\caption{Average TPR, FDP. (std. devs) for balanced neuronal network simulations with oracle tuning, averaged over 5 replicates. Best performing methods are boldfaced.}
\label{tab:bn}
\bigskip
\begin{footnotesize}
\begin{tabular}{|l|r|r|r|r|}
    \cline{1-3}
    & \multicolumn{2}{|c|}{Baseline}   \\
    \cline{1-3}
    \textbf{Model} &TPR&FDP \\
    \cline{1-3}
    Extreme (4) & 0.690 (0.060) & 0.303 (0.068) \\
    Extreme (6) & 0.751 (0.062) & 0.244 (0.063) \\
    Extreme (8) & \textbf{0.782} (0.067) & \textbf{0.205} (0.070)  \\
    \cline{1-3}
    Gaussian Glasso & 0.411 (0.068) & 0.582 (0.071)  \\
    Gaussian NS & 0.395 (0.065) & 0.604 (0.062) \\
    \cline{1-3}
    Quantile (0.5)  & 0.066 (0.022) & 0.940 (0.017) \\
    Quantile (0.9) & 0.506 (0.067) & 0.494 (0.070) \\
    Quantile (0.99) & 0.650 (0.072) & 0.339 (0.079) \\
    Quantile (0.999) & 0.524 (0.076) & 0.475 (0.074)  \\
    \hline
    & \multicolumn{2}{|c|}{$p = 300$} & \multicolumn{2}{|c|}{$p = 500$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & 0.578 (0.070) & 0.423 (0.068) & 0.452 (0.073) & 0.551 (0.070) \\
    Extreme (6) & 0.624 (0.074) & 0.373 (0.077) & 0.533 (0.078) & 0.462 (0.072)  \\
    Extreme (8) & \textbf{0.697} (0.072) & \textbf{0.299} (0.071) & \textbf{0.591} (0.079) & \textbf{0.407} (0.079)  \\
    \hline
    Gaussian Glasso & 0.376 (0.062) & 0.623 (0.063) & 0.302 (0.065) & 0.699 (0.068)  \\
    Gaussian NS & 0.349 (0.061) & 0.653 (0.064) & 0.263 (0.059) & 0.734 (0.062) \\
    \hline
    Quantile (0.5) & 0.050 (0.015) & 0.952 (0.018) & 0.055 (0.018) & 0.944 (0.016)  \\
    Quantile (0.9) & 0.451 (0.065) & 0.552 (0.062) & 0.426 (0.061) & 0.575 (0.064) \\
    Quantile (0.99) & 0.589 (0.072) & 0.411 (0.074) & 0.536 (0.076) & 0.465 (0.076) \\
    Quantile (0.999) & 0.533 (0.071) & 0.469 (0.075) & 0.497 (0.077) & 0.502 (0.078) \\
    \hline
    & \multicolumn{2}{|c|}{$0.0005 Hz$} & \multicolumn{2}{|c|}{$0.002 Hz$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & 0.804 (0.068) & 0.198 (0.065) & 0.463 (0.062) & 0.539 (0.069)  \\
    Extreme (6) & 0.832 (0.069) & 0.170 (0.060)  & 0.547 (0.065) & 0.464 (0.063) \\
    Extreme (8) & \textbf{0.855} (0.074) & \textbf{0.147} (0.071) &  \textbf{0.611} (0.071) & \textbf{0.392} (0.069)  \\
    \hline
    Gaussian Glasso & 0.399 (0.061) & 0.599 (0.057) & 0.444 (0.067) & 0.551 (0.062)\\
    Gaussian NS & 0.383 (0.053) & 0.620 (0.059)  & 0.426 (0.067) & 0.568 (0.066)  \\
    \hline
    Quantile (0.5) & 0.051 (0.028) & 0.947 (0.021) & 0.087 (0.019) & 0.914 (0.020) \\
    Quantile (0.9) & 0.602 (0.072) & 0.390 (0.070) & 0.351 (0.072) & 0.653 (0.069)  \\
    Quantile (0.99)  & 0.725 (0.076) & 0.279 (0.077) & 0.439 (0.073) & 0.559 (0.074) \\
    Quantile (0.999) & 0.594 (0.072) & 0.408 (0.075) & 0.433 (0.079) & 0.571 (0.077) \\
    \hline
    & \multicolumn{2}{|c|}{$\mu = 12$} & \multicolumn{2}{|c|}{$\mu = 16$} \\
    \hline
    \textbf{Model} &TPR&FDP &TPR&FDP\\
    \hline
    Extreme (4) & 0.411 (0.062) & 0.586 (0.065) & 0.476 (0.066) & 0.524 (0.071) \\
    Extreme (6) & 0.452 (0.060) & 0.549 (0.069) & 0.527 (0.069) & 0.485 (0.073) \\
    Extreme (8) & \textbf{0.468} (0.068) & \textbf{0.539} (0.071) & \textbf{0.587} (0.064) & \textbf{0.412} (0.067) \\
    \hline
    Gaussian Glasso & 0.322 (0.065) & 0.671 (0.067)  & 0.368 (0.067) & 0.641 (0.068) \\
    Gaussian NS & 0.311 (0.070) & 0.684 (0.069) & 0.344 (0.062) & 0.658 (0.065)  \\
    \hline
    Quantile (0.5) & 0.045 (0.012) & 0.944 (0.010) & 0.052 (0.011) & 0.952 (0.012) \\
    Quantile (0.9) & 0.323 (0.065) & 0.682 (0.072) & 0.437 (0.071) & 0.565 (0.064) \\
    Quantile (0.99) & 0.318 (0.074) & 0.584 (0.073) & 0.479 (0.078) & 0.521 (0.079) \\
    Quantile (0.999) & 0.278 (0.077) & 0.726 (0.071) & 0.415 (0.072) & 0.582 (0.073) \\
    \hline
\end{tabular}

\end{footnotesize}
\end{table}

The numerical results from the simulation study are shown in Table \ref{tab:bn}. As a whole, we see that the Subbotin graphical model does does the best in terms of estimating the true graph structure of the balanced network. The true positive and false discovery rates for the Subbotin graphical model are notably better than any of the other competing models; only the quantile graphical model at the 99th percentile is close. Interestingly, the quantile graphical model at the 99.9th percentile actually performs worse than at the 99th percentile. This highlights that, for analyzing extreme values, the selection of quantile can have a large impact on the resulting graphical model estimate and that choosing the correct quantile is not simply a question of choosing as large of a quantile as computationally possible. We also note the median quantile graphical model performs particularly poorly in this set of simulations because it is more robust to rare extreme values relative to the Gaussian or Subbotin graphical model by design, meaning that it puts even less relative weight on the extreme values when performing parameter estimation. As expected, increasing the number of simulated neurons in the system decreases the accuracy of all methods. Also unsurprisingly, decreasing the average magnitudes of the simulated spikes decreases the performance of all methods with respect to finding the graph structure with respect to these observations. Interestingly, decreasing the number of spikes per neuron actually leads to better performance from all methods; this could be caused by a resulting decrease in the number of true edges of the graph as well as a smaller probability of finding a false positive match between a true extreme observation and a noise observation.
\end{comment}


\bibitem[\protect\citeauthoryear{Akil, Rosenbaum, and Josić}{2020}]{aa2}
Akil, A.E., Rosenbaum, R. and Josić, K. (2020).
Synaptic Plasticity in Correlated Balanced Networks.
{\em arXiv preprint arXiv:2004.12453.}





%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%




\begin{table}[t]
\caption{Average TPR, FDP. (std. dev.) for the multivariate Subbotin graphical model distribution simulations with oracle tuning, averaged over 50 replicates. Best performing methods are boldfaced.}
\label{tab:mvgn}
\medskip
\begin{footnotesize}
\begin{tabular}{|l|r|r|r|r|}
    \cline{1-3}
    & \multicolumn{2}{|c|}{Baseline}  \\
    \cline{1-3}
    \textbf{Model} &TPR&FDP \\
    \cline{1-3}
    Subbotin (4) & 0.793 (0.058) &  0.205 (0.059)  \\
    Subbotin (6) & 0.812 (0.054) &  0.200 (0.050) \\
    Subbotin (8) & \textbf{0.840} (0.052) &  \textbf{0.166} (0.053) \\
    \cline{1-3}
    Gaussian NS & 0.779 (0.061) & 0.215 (0.059) \\
    Gaussian Glasso & 0.411 (0.068) & 0.582 (0.071)  \\
    \cline{1-3}
    Quantile (0.5)  & 0.689 (0.075) & 0.223 (0.079) \\
    Quantile (0.9) & 0.277 (0.083) & 0.727 (0.087)\\
    \cline{1-3}
    Copula (10) & 0.552 (0.056) & 0.457 (0.054) \\
    Copula (20) & 0.511 (0.046) & 0.489 (0.043) \\
    Copula (30) & 0.543 (0.050) & 0.454 (0.049) \\
    \hline
     & \multicolumn{2}{|c|}{$n = 1000$} & \multicolumn{2}{|c|}{$n = 4000$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Subbotin (4) & 0.534 (0.058) &  0.469 (0.059) & 0.853 (0.052) & 0.150 (0.054) \\
    Subbotin (6) & 0.564 (0.062) &  0.441 (0.060) & 0.859 (0.051) & 0.142 (0.053) \\
    Subbotin (8) & \textbf{0.631} (0.055) &  \textbf{0.367} (0.053) & \textbf{0.893} (0.055) & \textbf{0.105} (0.055) \\
    \hline
    Gaussian NS & 0.503 (0.059) & 0.490 (0.059) & 0.863 (0.048) & 0.125 (0.047)\\
    Gaussian Glasso & 0.376 (0.062) & 0.623 (0.063) & 0.302 (0.065) & 0.699 (0.068)  \\
    \hline
    Quantile (0.5) & 0.482 (0.079) & 0.520 (0.075) & 0.817 (0.071) & 0.172 (0.073)\\
    Quantile (0.9) & 0.259 (0.081) & 0.744 (0.084)& 0.345 (0.077) & 0.652 (0.075)\\
    \hline
    Copula (10) & 0.534 (0.056) & 0.465 (0.052) & 0.535 (0.045) & 0.463 (0.048) \\
    Copula (20) & 0.521 (0.052) & 0.478 (0.054) & 0.517 (0.046) & 0.485 (0.045) \\
    Copula (30) & 0.500 (0.054) & 0.499 (0.050) & 0.521 (0.043) & 0.477 (0.044) \\
    \hline 
    & \multicolumn{2}{|c|}{$p = 300$} & \multicolumn{2}{|c|}{$p = 1000$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Subbotin (4) & 0.684 (0.058) &  0.311 (0.056) & 0.503 (0.059) &  0.501 (0.060)  \\
    Subbotin (6) & 0.732 (0.059) &  0.272 (0.055) & \textbf{0.563} (0.053) & \textbf{0.438} (0.056) \\
    Subbotin (8) & \textbf{0.751} (0.056) &  \textbf{0.250} (0.054) & 0.545 (0.061) &  0.452 (0.055)  \\
    \hline
    Gaussian NS & 0.634 (0.053) & 0.362 (0.056) & 0.471 (0.057) & 0.507 (0.055) \\
    Gaussian Glasso & 0.399 (0.061) & 0.599 (0.057) & 0.444 (0.067) & 0.551 (0.062)\\
    \hline
    Quantile (0.5) & 0.573 (0.078) & 0.427 (0.081) & 0.416 (0.077) & 0.590 (0.078)  \\
    Quantile (0.9) & 0.265 (0.085) & 0.747 (0.085) & 0.284 (0.079) & 0.731 (0.082) \\
    \hline
    Copula (10) & 0.524 (0.050) & 0.477 (0.055) & 0.460 (0.059) & 0.541 (0.060) \\
    Copula (20) & 0.525 (0.053) & 0.478 (0.053) & 0.449 (0.061) & 0.550 (0.063) \\
    Copula (30) & 0.521 (0.057) & 0.419 (0.055) & 0.451 (0.058) & 0.551 (0.061) \\
    \hline
    & \multicolumn{2}{|c|}{$\nu = 4$} & \multicolumn{2}{|c|}{$\nu = 6$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Subbotin (4) & \textbf{0.886} (0.053) &  \textbf{0.107} (0.054) & 0.823 (0.060) &  0.170 (0.059)  \\
    Subbotin (6) & 0.842 (0.057) &  0.158 (0.055) & \textbf{0.855} (0.057) &  \textbf{0.137} (0.057)  \\
    Subbotin (8) & 0.734 (0.062) &  0.261 (0.058) & 0.775 (0.051) &  0.218 (0.058) \\
    \hline
    Gaussian NS & 0.865 (0.053) & 0.134 (0.050) & 0.779 (0.051) & 0.225 (0.059)  \\
    Gaussian Glasso & 0.322 (0.065) & 0.671 (0.067)  & 0.368 (0.067) & 0.641 (0.068) \\
    \hline
    Quantile (0.5) & 0.664 (0.072) & 0.335 (0.073)  & 0.626 (0.072) & 0.381 (0.079)  \\
    Quantile (0.9) & 0.252 (0.079) & 0.776 (0.081) & 0.250 (0.080) & 0.746 (0.083) \\
    \hline
    Copula (10) & 0.565 (0.055) & 0.433 (0.052) & 0.553 (0.053) & 0.445 (0.055) \\
    Copula (20) & 0.553 (0.049) & 0.447 (0.051) & 0.537 (0.046) & 0.465 (0.048) \\
    Copula (30) & 0.551 (0.051) & 0.447 (0.054) & 0.529 (0.052) & 0.471 (0.057) \\
    \hline
\end{tabular}
\end{footnotesize}
\end{table}





%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%





\begin{table}[H]
\caption{Average TPR, FDP. (std. devs) for multivariate extreme graphical model distribution simulations with stability selection, averaged over 5 replicates. Best performing methods are boldfaced.}
\bigskip
\begin{footnotesize}
\begin{tabular}{|l|r|r|r|r|}
    \cline{1-3}
    & \multicolumn{2}{|c|}{Baseline} \\
    \cline{1-3}
    \textbf{Model} &TPR&FDP \\
    \cline{1-3}
    Extreme (4) & 0.783 (0.072) & 0.267 (0.070)  \\
    Extreme (6) & 0.826 (0.075) & 0.269 (0.064) \\
    Extreme (8) & \textbf{0.855} (0.069) & \textbf{0.257} (0.072) \\
     \cline{1-3}
    Gaussian Glasso & 0.761 (0.072) & 0.353 (0.069)\\
    Gaussian NS & 0.744 (0.068) & 0.369 (0.062) \\
     \cline{1-3}
    Quantile (0.5) & 0.624 (0.065) & 0.355 (0.069) \\
    Quantile (0.9) & 0.258 (0.063) & 0.730 (0.068) \\
    \hline
     & \multicolumn{2}{|c|}{$n = 1000$} & \multicolumn{2}{|c|}{$n = 4000$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & 0.529 (0.079) & 0.549 (0.066) & 0.842 (0.065) & 0.229 (0.064)\\
    Extreme (6) & 0.555 (0.072) & 0.542 (0.061) & 0.854 (0.073) & \textbf{0.226} (0.065)  \\
    Extreme (8) & \textbf{0.623} (0.075) & \textbf{0.501} (0.067) & \textbf{0.878} (0.071) & 0.235 (0.067)  \\
    \hline
    Gaussian Glasso & 0.484 (0.072) & 0.571 (0.069) & 0.852 (0.062) & 0.270 (0.069)  \\
    Gaussian NS & 0.491 (0.077) & 0.554 (0.082) & 0.823 (0.062) & 0.266 (0.065)\\
    \hline
    Quantile (0.5) & 0.466 (0.068) & 0.582 (0.080) & 0.817 (0.077) & 0.250 (0.071)\\
    Quantile (0.9) & 0.223 (0.067) & 0.771 (0.062) & 0.301 (0.067) & 0.697 (0.064) \\
    \hline
    & \multicolumn{2}{|c|}{$p = 300$} & \multicolumn{2}{|c|}{$p = 1000$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & 0.636 (0.079) & 0.343 (0.074) & 0.478 (0.077) & 0.586 (0.065) \\
    Extreme (6) & 0.697 (0.075) & 0.379 (0.072) & \textbf{0.545} (0.071) & 0.527 (0.063) \\
    Extreme (8) & \textbf{0.708} (0.068) & \textbf{0.366} (0.065) & 0.536 (0.071) & \textbf{0.517} (0.070)\\
    \hline
    Gaussian Glasso & 0.627 (0.073) & 0.506 (0.074) & 0.439 (0.077) & 0.692 (0.078) \\
    Gaussian NS & 0.651 (0.068) & 0.463 (0.071) & 0.457 (0.073) & 0.629 (0.072) \\
    \hline
    Quantile (0.5) & 0.551 (0.065) & 0.539 (0.069)  & 0.424 (0.072) & 0.677 (0.070)  \\
    Quantile (0.9) & 0.224 (0.055) & 0.780 (0.060) & 0.109 (0.052) & 0.923 (0.054) \\
    \hline
    & \multicolumn{2}{|c|}{$\nu = 4$} & \multicolumn{2}{|c|}{$\nu = 6$} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & \textbf{0.906} (0.045) &  \textbf{0.197} (0.059) & 0.815 (0.061) &  0.270 (0.062)  \\
    Extreme (6) & 0.859 (0.051) &  0.244 (0.058) & \textbf{0.876} (0.057) &  \textbf{0.147} (0.056)  \\
    Extreme (8) & 0.757 (0.061) &  0.271 (0.060) & 0.764 (0.067) &  0.338 (0.063) \\
    \hline
    Gaussian Glasso & 0.855 (0.072) & 0.197 (0.067) & 0.811 (0.065) & 0.284 (0.067)  \\
    Gaussian NS & 0.836 (0.068) & 0.198 (0.065) & 0.824 (0.062) & 0.279 (0.063)  \\
    \hline
    Quantile (0.5) & 0.620 (0.076) & 0.416 (0.061) & 0.617 (0.067) & 0.409 (0.077) \\
    Quantile (0.9) & 0.287 (0.062) & 0.721 (0.068) & 0.232 (0.064) & 0.776 (0.057) \\
    \hline
    & \multicolumn{2}{|c|}{Chain} & \multicolumn{2}{|c|}{Erdos-Renyi} \\
    \hline
    \textbf{Model} &TPR&FDP&TPR&FDP\\
    \hline
    Extreme (4) & 0.652 (0.064) & 0.357 (0.078)  & \textbf{0.623} (0.077) & \textbf{0.426} (0.073) \\
    Extreme (6) & 0.667 (0.072) & 0.355 (0.077) & 0.601 (0.070) & 0.454 (0.078)\\
    Extreme (8) & \textbf{0.695} (0.075) & \textbf{0.312} (0.077) & 0.608 (0.078) & 0.450 (0.071)  \\
    \hline
    Gaussian Glasso & 0.606 (0.071) & 0.486 (0.069) & 0.571 (0.073) & 0.456 (0.074) \\
    Gaussian NS & 0.587 (0.079) & 0.480 (0.078) & 0.574 (0.061) & 0.457 (0.077) \\
    \hline
    Quantile (0.5) & 0.550 (0.073) & 0.455 (0.071) & 0.534 (0.075) & 0.475 (0.069) \\
    Quantile (0.9) & 0.182 (0.051) & 0.790 (0.060) & 0.191 (0.054) & 0.788 (0.058) \\
    \hline
\end{tabular}
\end{footnotesize}
\end{table}



\begin{comment}
Instead of using a full likelihood of the joint graphical model distribution, we combine feature selection estimates for the node-wise conditional distributions in order to estimate the graph structure. For each individual node $x_i$, we can estimate its graph neighborhood, defined as the minimal set such that $x_i$ is conditionally independent of all remaining variables, by applying a generalized linear regression model predicting $x_i$ from all other variables in the data set. An $\ell_1$ regularization penalty is added to the regression problem in order to induce sparsity in the selected number of relevant features. After estimating the individual neighborhoods, the node-wise parameter estimates can be fused together to create a single graph estimate by selecting as the edge set for the graph all pairs of nodes which have a non-zero linear relationship with one another in both directions, i.e. all cases where a node $x_i$ is considered to be a neighbor of $x_j$ and $x_j$ is considered to be a neighbor of $x_i$. Alternatively, we can select as neighbors all pairs of nodes which have a non-zero linear relationship with one another in only one direction, i.e. cases where a node $x_i$ is considered to be a neighbor of $x_j$ or $x_j$ is considered to be a neighbor of $x_i$, but not necessarily both. As has been shown in previous literature, these two schemes will be asymptotically equivalent \citep{nm1}.

and the parameters for the regression problem can be estimated using the algorithmic procedure outlined in the aforementioned paper.
\end{comment}


\begin{comment} 


With modern calcium imaging technology, the activities of thousands of neurons can be recorded simultaneously. These experiments can potentially provide new insights into functional connectivity, defined as the statistical relationships between the activity of neurons in the brain. As a common tool for estimating conditional dependencies in high-dimensional settings, graphical models are a natural choice for analyzing calcium imaging data. However, raw neuronal activity data presents a unique challenge: the important information lies in rare extreme value observations that indicate neuronal firing. To address this issue, we develop a novel class of graphical models, called the Subbotin graphical model, which finds relationships between features with respect to the extreme values. Our model assumes the conditional distributions a subclass of the generalized normal or Subbotin distribution, and yields a form of a curved exponential family graphical model. We first derive the form of the Subbotin graphical model and show the conditions under which it is normalizable. We then demonstrate the model selection consistency of our estimation method. Lastly, we study the empirical performance of the Subbotin graphical model through several simulation studies, as well as a real data example in which we apply our method to a calcium imaging data set.
\end{comment}

